$C^1$ Robust Rigidity for Bi-critical Circle Maps

We prove that two topologically conjugate bi-critical circle maps whose signatures are the same, and whose renormalizations converge together exponentially fast in the $C^2$-topology, are $C^1$ conjugate.

==> Lemma5.5.tex <==
	\begin{lemma}\label{lema_pasocero} There exists $C_1 > 0$ and $\lambda_1=\lambda_1(\lambda, d) \in (0,1)$ such that for all $m<n+1$ we have:
	\begin{equation*}
		\max_{z  \in \widehat{E}_{n+1} \cap J_m} \left| B_{m,g} (h(z))- B_{m,f} (z)\right| \leq C_1 \left(\max_{z  \in \widehat{E}_{n+1} \cap J_{m+1}} \left| B_{m+1,g} (h(z))- B_{m+1,f} (z)\right| + \lambda_1^{m/2} \right).
	\end{equation*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lema_pasocero}]
	Let $m \leq n$, then by real bounds, the exponential converge of the renormalizations and the relation $B_{m,f}(t)= 
	-B_{m+1,f}(t) \mathcal{R}^{m}f(0)$, for  $t \in J_{m+1}$, we obtain that for $z  \in \widehat{E}_{n+1} \subset J_{m+1}$ then   		%With this at hand we observe that
	%{\small
		%	\begin{align*}
			%		&|B_{n,f}(f^{q_n}(c_0)) - B_{n,g}(g^{q_n}(c_0)) |
			%		= \left| \frac{-B_{n-1,f}(f^{q_n}(c_0)) }{\mathcal{R}^{n-1}f(0)} + \frac{B_{n-1,g}(g^{q_n}(c_0))}{ \mathcal{R}^{n-1}g(0)}  \right|\\
			%		&\leq \frac{|B_{n-1,g}(g^{q_n}(c_0)) - B_{n-1,f}(f^{q_n}(c_0)) |}{|\mathcal{R}^{n-1}f(0)|} 	 +
			%		|B_{n-1,g}(g^{q_n}(c_0))| \left| \frac{1}{\mathcal{R}^{n-1}g(0)} - \frac{1}{\mathcal{R}^{n-1}f(0)}\right|,
			%	\end{align*}
		%}
	%and using the exponential convergence of the renormalizations we have
	%{\small
		%	\begin{align*}
			%		|B_{n-1,g}(g^{q_n}(&c_0)) - B_{n-1,f}(f^{q_n}(c_0)) |
			%		\\ &= | \mathcal{R}^{n-1}g(0) \mathcal{R}^n g(0)B_{n+1,g}(g^{q_n}(c_0))-
			%		\mathcal{R}^{n-1}f(0) \mathcal{R}^n(0)B_{n+1,f}(f^{q_n}(0))  |\\
			%		&\leq |\mathcal{R}^{n-1}g(0) \mathcal{R}^{n}g(0)| \,  	|B_{n+1,g}(g^{q_n}(c_0)) - B_{n+1,f}(f^{q_n}(c_0)) | \\
			%		&+
			%		|B_{n+1,f}(f^{q_n}(c_0))| |\mathcal{R}^{n-1}g(0) \mathcal{R}^ng(0) - \mathcal{R}^{n-1}f(0) \mathcal{R}^nf(0)| \\
			%		&\leq C\, |B_{n+1,g}(g^{q_n}(c_0)) - B_{n+1,f}(f^{q_n}(c_0)) | \, + \, C\, \lambda^{n}.
			%	\end{align*}
		%}
	%so, putting the last inequalities together we obtain
	\begin{align*}\label{ine:estimatesextremesqn}
		\left|B_{m,f}(z) - B_{m,g}(h(z)) \right| &\leq 
		C\, \lambda^m + C \, |B_{m+1,f}(z)- B_{m+1,g}(h(z))| \\
		&\leq C \left( \lambda^m + \max_{v \in \widehat{E}_{n+1} \cap J_{m+1}} |B_{m+1,g}(h(v)) - B_{m+1,f}(v)| \right).
	\end{align*}
	%	and  therefore % for all $z  \in \widehat{E}_{n+1} \cap J_{m+1}$ 	
	%	{\small
		%		\begin{equation}\label{ine:estimatesextremesqn+2}
			%			\left|B_{m,f}(f^{q_{n+2}}(c_0)) - B_{m,g}(g^{q_{n+2}}(c_0)) \right| 
			%&= | - B_{n+1,f}(f^{q_{n+2}}(c_0)) \mathcal{R}^{n}f(0) + B_{n+1,g}(g^{q_{n+2}}(c_0)) \mathcal{R}^n g(0) | \\
			%&\leq | - B_{n+1,f}(f^{q_{n+2}}(c_0)) \mathcal{R}^{n}f(0) + B_{n+1,f}(f^{q_{n+2}}(c_0)) \mathcal{R}^n g(0) | \\
			%	&+ | B_{n+1,g}(g^{q_{n+2}}(c_0)) \mathcal{R}^{n}g(0) - B_{n+1,f}(f^{q_{n+2}}(c_0)) \mathcal{R}^n g(0) | \\
			%&\leq |\mathcal{R}^{n}g(0)- \mathcal{R}^{n}f(0)| \,  	|B_{n+1,f}(f^{q_{n+2}}(c_0))| + |\mathcal{R}^ng(0)| |B_{n+1,g}(g^{q_{n+2}}(c_0))- B_{n+1,f}(f^{q_{n+2}}(c_0))|\\
			%		\leq C\, \lambda^m + C \, |B_{m+1,g}(g^{q_{n+2}}(c_0))- B_{m+1,f}(f^{q_{n+2}}(c_0))|.
			%	\end{equation}
		%}
	%	From inequalities \eqref{ine:estimatesextremesqn}, \eqref{ine:estimatesextremesqn+2} and  \eqref{ine:estimatefreakc}, we have the following three estimates for all $m \leq n$:
	%	\begin{align}\label{inq:estimativaprimerosextremos}
		%	|B_{m,f}(z) - B_{m,g}(h(z)) |
		%	\leq C \left( \lambda^m + \max_{v \in \widehat{E}_{n+1} \cap J_{m+1}} |B_{m+1,g}(h(v)) - B_{m+1,f}(v)| \right).
		%\end{align}
		So we just need to prove the result for $z  \in \widehat{E}_{n+1} \cap (J_m \setminus J_{m+1})$ and $m< n+1$. If $z=f^{q_m}(c_0)$ or $z=f^{q_{m+2}}(c_0)$ then $z$ satisfies the lemma for $\lambda= \lambda_1$ since by
		%{\small
			%	\begin{align*}\label{inq:estimativaultimosextremos}
				%	|B_{m,f}(f^{q_{m}}(z)) - B_{m,g}(g^{q_{m}}(z)) |
				%	\leq S_1 \left( \lambda^m + \max_{v \in \widehat{E}_{n+1} \cap J_m} |B_{m+1,g}(h(v)) - B_{m+1,f}(v)| \right)
				%\end{align*}
				%}
			%	and
			%	\begin{align}\label{inq:estimativafree}
				%	|B_{m,f}(\mathfrak{c}_{n}^f) - B_{m,g}(\mathfrak{c}_{n}^g) |
				%	\leq S_1 \left( \lambda^{m} + \max_{v \in \widehat{E}_{n+1} \cap J_m} |B_{m+1,g}(h(v)) - B_{m+1,f}(v)| \right).
				%\end{align}
				by the convergence of renormalizations  we have
				\begin{equation}\label{ineq:estimativaBmfqm}
					|B_{m,f}(u) - B_{m,g}(h(u))| \leq  C\,\lambda^{m}.
				\end{equation}
				Moreover, by Inequality \eqref{eq:diferenciafreecriticalpoint}, $\mathfrak{c}_{m} \in \widehat{E}_{n+1}$ also satisfies the lemma for $\lambda_1=\lambda^{1/d}$.
				Let  %We will show that the vertices of  $\widehat{E}_{m+1}$ which are backwards iterates of $\mathfrak{c}_{m}^f$, by $\mathcal{R}^{m}f$, and the vertices that are forward iterates of $f^{q_m}(c_0)$, by $\mathcal{R}^{m}f$, also satisfy the lemma. The other points of $\widehat{E}_{m+1}$ will satisfy the lemma with an analogous argument.
				\textcolor{blue}{$N = \lfloor \frac{2}{L_2} \rfloor +1$}. If $a_{m+1} \leq N$, then by finite induction % using that  $f^{q_m}(c_0)$ and $\mathfrak{c}_{m}^f$ satisfy the lemma, real bounds (Theorem \ref{teobeau}), Corollary \ref{c1bounds} and Lemma \ref{lemma:derivadameanvaluethrm}, 
				we obtain the lemma for $\widehat{E}_{m+1} \subset J_m$. Otherwise, if $a_{m+1} > N$, then for each $0 \leq i \leq N$ let $\theta_i \in (B_{m,f}(f^{q_m+iq_{m+1}}(c_0)), B_{m,g}(g^{q_m+iq_{m+1}}(c_0)))$, given by Mean Value Theorem, such that
				\begin{align*}
					|B_{m,f}(f^{q_m+(i+1)q_{m+1}}(c_0)) &- \mathcal{R}^mf(B_{m,g}(g^{q_m+iq_{m+1}}(c_0)))| \\ 
					&=  |D\mathcal{R}^mf(\theta_i)| \, |B_{m,f}(f^{q_m+iq_{m+1}}(c_0))- B_{m,g}(g^{q_n+iq_{m+1}}(c_0))|.
				\end{align*} 
				By Inequality \eqref{ineq:estimativaBmfqm} and Corollary  \ref{c1bounds}, for all $0 \leq i \leq N$,   we have:
				\begin{align*}
					&|B_{m,f}(f^{(i+1)q_{m+1}+q_m}(c_0))- B_{m,g}(g^{(i+1)q_{m+1}+q_m}(c_0))| \\ 
					&\leq  |D\mathcal{R}^mf(\theta_i)| \, |B_{m,f}(f^{iq_{m+1}+q_m}(c_0))- B_{m,g}(g^{iq_{m+1}+q_m}(c_0))|\\
					&\hspace{1.8cm}+
					| \mathcal{R}^mf(B_{m,g}(g^{iq_{m+1}+q_m}(c_0)))-
					\mathcal{R}^mg(B_{m,g}(g^{iq_{m+1}+q_m}(c_0)))|\\
					&\leq \dots \leq |D\mathcal{R}^mf(\theta_i)| \cdots |D\mathcal{R}^mf(\theta_0)| \, |B_{m,f}(f^{q_m}(c_0))- B_{m,g}(g^{q_m}(c_0))| + i \ C\, \lambda^m\\
					%&\leq  K^N\, \left( \max_{v \in \widehat{E}_{n+1} \cap J_m} |B_{m+1,g}(v) - B_{m+1,f}(h(v))| \right) + (K^N+iC)\, \lambda^{m}\\
					&\leq  K^N\, \left( \max_{v \in \widehat{E}_{m+1} \cap J_m} |B_{m+1,g}(h(v)) - B_{m+1,f}(v)| \right) + (K^N+NC)\, \lambda^{m}.
				\end{align*}
				Analogously,  let $\Theta_i \in (B_{m,f}(f^{-iq_{m+1}}(\mathfrak{c}_{m}^f)), B_{m,g}(g^{-iq_{m+1}}(\mathfrak{c}_{m}^g)))$ such that
				\begin{align*}
					|B_{m,f}(f^{(-i+1)q_{m+1}}(\mathfrak{c}_{m}^f)) &- (\mathcal{R}^mf)(B_{m,g}(g^{-iq_{m+1}}(\mathfrak{c}_{m}^g)))| \\ 
					&=  |D\mathcal{R}^mf(\Theta_i)| \, |B_{m,f}(f^{-iq_{m+1}}(\mathfrak{c}_{m}^f))- B_{m,g}(g^{-iq_{m+1}}(\mathfrak{c}_{m}^g))|.
				\end{align*}
				Again, by \eqref{ineq:estimativaBmfqm} and Corollary  \ref{c1bounds}:
				\begin{align*}
					&|B_{m,f}(f^{-(i+1)q_{m+1}}(\mathfrak{c}_{m}^f))- B_{m,g}(g^{-(i+1)q_{m+1}}(\mathfrak{c}_{m}^g))| \\ 
					%	&\leq  |(\mathcal{R}^mf)'(\Theta_i)|^{-1} \, |B_{m,f}(f^{-(i-1)q_{m+1}}(\mathfrak{c}_{m}^f))- B_{m,g}(g^{-(i-1)q_{m+1}}(\mathfrak{c}_{m}^g))|\\
					%	&\hspace{1.5cm}+  |(\mathcal{R}^mf)'(\Theta_i)|^{-1}| \ | \mathcal{R}^mf(B_{m,g}(g^{-iq_{m+1}}(\mathfrak{c}_{m}^g))-
					%	\mathcal{R}^mg(B_{m,g}(g^{-iq_{m+1}}(\mathfrak{c}_{m}^g)))|\\
					%	&\leq \dots \leq |(\mathcal{R}^mf)'(\Theta_i)|^{-1} \cdots |(\mathcal{R}^mf)'(\Theta_0)|^{-1} \, |B_{m,f}(\mathfrak{c}_{m}^f)- B_{m,g}(\mathfrak{c}_{m}^g)| +  i \ C\, \lambda^{m/d}\\
					%	&\leq K^{N} \left( \max_{v \in \widehat{E}_{n+1} \cap J_m} |B_{m+1,f}(v) - B_{m+1,g}(h(v))| + \lambda_{1}^{m} \right) + K\, C \, N\, \lambda_1^{m} \\
					&\hspace{2.3cm}\leq K^{N} \left( \max_{v \in \widehat{E}_{m+1} \cap J_m} |B_{m+1,f}(v) - B_{m+1,g}(h(v))| \right) +  (K\, C \, N\, + K^{N}) \lambda^{m/d}.
				\end{align*}
				We repeat the process above this time replacing $\mathfrak{c}_{m}$ by $f^{q_{m+2}}(c_0)$, and $f^{q_{m}}(c_0)$ by $\mathfrak{c}_{m}$.
				For all those endpoints the lemma follows taking $S_1=K^N+KCN$ and $\lambda_1=\lambda^{1/d}$.  Let $P= \lfloor \frac{1}{\lambda} \rfloor +1$ and consider the next $P$ points in $\widehat{E}_{m+1}$. We have two options, or we had covered all  endpoints  (which implies that $r(m)$ and $\ell(m)$ are both smaller than $P+N$) or we still have more endpoints to cover. \textcolor{red}{In the first case, the tubulars  $M_{m,L_2}^f$ and $M_{m,L_2}^g$ \textcolor{red}{creo que es $N+P$ en lugar de $L_2$} are non-empty. For all $z \in M_{m,L_2}^f \cap M_{m,L_2}^g$ we have $|(\mathcal{R}^mf)'(z)|<1 $ and $|(\mathcal{R}^mf)'(z)|^{-1}<1$, hence for $N+2 \leq j \leq P$,} we have
				\begin{align*}
					&|B_{m,f}(f^{(j+1)q_{m+1}}(c_0))- B_{m,g}(g^{(j+1)q_{m+1}}(c_0))| \\ 
					&\leq  \dots \leq |B_{m,f}(f^{(N+1)q_{m+1}}(c_0))- B_{m,g}(g^{(N+1)q_{m+1}}(c_0))| + (K^N+KCN)P\, \lambda^{m}\\
					&\leq  (K^N+KCN)\, \left( \max_{v \in \widehat{E}_{n+1} \cap J_m} |B_{m+1,g}(h(v)) - B_{m+1,f}(v)|  \ + \ \left(\frac{1}{\lambda} +1 \right)\, \lambda^{m}\right),
				\end{align*}
				and analogously
				\begin{align*}
					&|B_{m,f}(f^{-jq_{m+1}}(\mathfrak{c}_{m}^f))- B_{m,g}(g^{-jq_{m+1}}(\mathfrak{c}_{m}^g))| \\ 
					%	&\leq  \dots \leq |B_{m,f}(f^{-(N+1)q_{m+1}}(\mathfrak{c}_{m}^f)))- B_{m,g}(g^{-(N+1)q_{m+1}}(\mathfrak{c}_{m}^g)))| +  (K^N+KCN)M\, \lambda^{m}\\
					&\leq   (K^N+KCN)\, \left( \max_{v \in \widehat{E}_{n+1} \cap J_m} |B_{m+1,g}(h(v)) - B_{m+1,f}(v)| \ +  \ \left( \frac{1}{\lambda} +1 \right)\, \lambda^{m/d}\right),
				\end{align*}
				Similarly, we get the same inequality  replacing $\mathfrak{c}_{m}$ by $f^{q_{m+2}}(c_0)$, and  $f^{q_{m}}(c_0)$ by $\mathfrak{c}_{m}$. We get the lemma in all those cases taking $S_1= \max\{ KCN+K^N, 2(KCN+K^N)\lambda^{-1} \}$ and $\lambda_1=\lambda^{1/d}$.\\
				If we still have more endpoints to cover (that means that  $r(m)-N>P$ or $\ell(m)-N>P$ or both, and in particular $a_{m+1}>P+N$), then the centers of the tubular $M_{m,N+P}^f$ is defined.
				%%%%%%%%%%%%%%%%%%%%%%%%%%
				
				
				\begin{claim}\label{claimP}
					Let  $n \geq m$, $P= \lfloor \frac{1}{\lambda} \rfloor +1$ and   $N = \lfloor \frac{2}{L} \rfloor +1$. If $a_{m+1}> N+P$ , then  there exists $C=C(\varepsilon,D_1,D_4, N,P, L_1, L_2, L_3,L_4)>0$  such that,
					\begin{equation*}
						|B_{m,f}(v)-z_{m}|< C\, \lambda^m %\frac{C}{P},
					\end{equation*}
					for all  $v \in	\widehat{E}_{n+1} \cap I_m$ with $v \in [f^{-Pq_{m+1}}(\mathfrak{c}_{m}) , f^{q_m+Pq_{m+1}}(c_0) ]$ if $r(m)>N+P$, or $v \in [f^{q_{m+2}-Pq_{m+1}}(c_0) , f^{Pq_{m+1}}(\mathfrak{c}_{m})]$ if $\ell(m)>N+P$.
				\end{claim}
				
				%\begin{lemma}
				%	Let $m \in \nt$ and $n \geq m$. If  $N \in \nt$ % = \lfloor \frac{2}{L_2} \rfloor +1$ este $L_2$ depende de $m$?)} and   	is such that $M_{m,N}^f$ is not empty and its center $z_{m,f}$ is defined then  there exists $C>0$ such that,  for $P= \lfloor \frac{1}{\lambda} \rfloor +1$, %(\textcolor{red}{En particular, $P$ es el mismo para todo $n$}). we have
			%	\begin{equation*}
				%		|B_{m,f}(f^{jq_{m+1}+q_m}(c_0))-z_{m,f}|< \frac{C}{P},
				%	\end{equation*}
			%	 for all  $P+1 \leq j \leq r(m)$  (if  $z_{m,f}$ is between  $\mathfrak{c}_{m}$ and $f^{q_{m}}(c_0)$), or for all  $-a_{m+1}+P \leq j \leq \ell(m)$  (if  $z_{m,f}$ is between $f^{q_{m+2}}(c_0)$ and $\mathfrak{c}_{m}$).
			%	Moreover, 
			%	\begin{equation*}
				%		|B_{m,f}(f^{-jq_{m+1}}(\mathfrak{c}_{m}))-z_{m,f}| < \frac{C}{P}.
				% 	\end{equation*} 
			%	 for $P \leq j\leq r(m)$ (if  $z_{m,f}$ is between  $\mathfrak{c}_{m}$ and $f^{q_{m}}(c_0)$), or for all  $-\ell(m) \leq j \leq -P $  (if  $z_{m,f}$ is between $f^{q_{m+2}}(c_0)$ and $\mathfrak{c}_{m}$).
			% \end{lemma}
		
		
		\begin{proof}[Proof of Claim \ref{claimP}]
			Since $a_{m+1}> N+P$, then one (or both) of the centers of $M_{m,N}^f$ is defined. Without lost of generality, let us assume that the center $z_{m}\in $. Let $\mathcal{F}$ be the tubular-coordinates  of $\mathcal{R}^mf$ with respect to $z_{m}$ (see Definition \ref{def:tubularcoordinates}). Observe that  $a_{m+1} \, ( z_{m} - \mathcal{R}^mf(z_{m})) <1$, then
			\begin{equation}\label{eq:varepsiloneM}
				0< -\varepsilon = -\mathcal{F}(0)
				< \frac{D^2\mathcal{R}^mf(z_{m,1})}{2\, a_{m+1}} <  %\frac{\|\mathcal{R}^mf \|_{C^2}}{2 (N+M)} <
				\frac{M}{2(N+P)}.
			\end{equation} 
			Let $i_c \in \nt$ be the smallest natural number such that $\mathcal{F}^{i_c}(\phi(1)) \in (0,-\varepsilon]$ and let $i_{r} \in \nt$ be such that  $\mathcal{F}^{i_{r}}(\phi(1))$ is the most right endpoint of the Funnel. Note that between $\mathcal{F}^{i_c}(\phi(1))$ and $\mathcal{F}^{i_{r}}(\phi(1))$ there are $B=\frac{1}{\sqrt{|\varepsilon|}} \tan^{-1}\left( \frac{1}{|\varepsilon|^{1/6}}\right)$ iterates.
			For the Funnel we use the estimates given by Lemma \ref{lemaKTfunnel} and for the Tunnel we use Lemma \ref{lemaKTtunnel}. 
			
			\textbf{Funnel:} Using Inequality \eqref{eq_funnelsis0} in Lemma \ref{lemaKTfunnel} for the map $\mathcal{F}^{-1}$, with $s_0=\mathcal{F}^{i_c}(\phi(1))$, $s_k=\mathcal{F}^{i_c-k}(\phi(1))$, and inequality \eqref{eq:varepsiloneM} we get, for all $0 \leq k$
			\begin{align*}
				|\mathcal{F}^{i_{r}-k}(\phi(1))| =|s_{i_c-i_{r}+k}|  &\leq
				\left|s_{i_c-i_{r}+k}- \frac{1}{i_c-i_{r}+k+ s_0^{-1} }\right| + \left|\frac{1}{i_c-i_{r}+k+ s_0^{-1}} \right|\\ 
				&\leq D_1 \left(\frac{s_0}{s_0(i_c-i_{r}+k)+1}\right)^{1+\alpha} + \frac{s_0}{s_0(i_c-i_{r}+k)+1} \\
				&\leq   -(D_1+1)\, \varepsilon \\
				&\leq \frac{M\,(D_1+1)}{2(P+N)}.
				%&\leq \frac{L_1\,(D_1+1)}{2}\, \lambda^{m}.
			\end{align*}
			
			%	\begin{align*}
				%		|\mathcal{F}^{i_{r}}(\phi(1))| =|s_{i_c-i_{r}}|  &\leq
				%		\left|s_{i_c-i_{r}}- \frac{1}{i_c-i_{r}+ s_0^{-1} }\right| + \left|\frac{1}{i_c-i_{r}+ s_0^{-1}} \right|\\ 
				%		&\leq D_1 \left(\frac{s_0}{s_0(i_c-i_{r})+1}\right)^{1+\alpha} + \frac{s_0}{s_0(i_c-i_{r})+1} \\
				%		&\leq   -(D_1+1)\, \varepsilon \\
				%		&\leq \frac{L_1\,(D_1+1)}{2(P+N)}. %= \frac{C}{P+N}.
				%	\end{align*}
			Since $|\frac{1}{2} (D^2\mathcal{R}^mf(z_{m})((\mathcal{R}^ m_f)^{i_{r}+k}(B_{m,f}(f^{q_m}(c_0)))- z_{m}) |=|\mathcal{F}^{i_{r}+k}(\phi(1))|$ then
			\begin{align*}
				|B_{m,f}(f^{(i_{r}+k)q_{m+1}+ q_m}(c_0))- z_{m}| = \left|(\mathcal{R}^m_f)^{(i_{r}+k)}(B_{m,f}(f^{q_m}(c_0)))- z_{m}\right|
				< \frac{M\,(D_1+1)}{2 K_3} \, \lambda^{m}.
			\end{align*} 
			%the claim follows for $B_{m,f}(f^{i_{\ell}q_{m+1}+q_m}(c_0))$. 
			Then we get the desired estimate in $|B_{m,f}(f^{iq_{m+1} +{q_m}}(c_0))- z_{m}|$, for  $N+P \leq i < i_{r}$.
			
			\textbf{Tunnel:} Now, we would like to etimative  $|B_{m,f}(f^{iq_{m+1} +{q_m}}(c_0))- z_{m,1}|$, for  $i_r \leq i \leq i_{c}$, that is, for $B=\frac{1}{\sqrt{|\varepsilon|}} \tan^{-1}\left( \frac{1}{|\varepsilon|^{1/6}}\right)$ iterates, in particular finite iterates. Applying Inequality \eqref{eq_tunnelsis0} in Lemma \ref{lemaKTtunnel} for $\mathcal{F}$, with  $|s_0|=|\mathcal{F}^{i_{r}}(\phi(1))| \leq -(1+D_1)\, \varepsilon$, we get that 
			\begin{align*}
				|\mathcal{F}^{i_{r}+1}(\phi(1))| =|s_1| \leq |s_{0}| - |s_0 -s_1| \leq -((1+D_1)+(1+D_4))\, \varepsilon \leq \frac{M\,((1+D_1)+(1+D_4))}{2(P+N)}.
			\end{align*}
			Therefore
			\begin{align*}
				|B_{m,f}(f^{(i_{r}+1)q_{m+1}+ q_m}(c_0))- z_{m}| =
				|(\mathcal{R}^ m_f)^{i_{r}+1}(B_{m,f}(f^{q_m}(c_0)))- z_{m}|
				< \frac{M\,((1+D_1)+(1+D_4))}{2(P+N)\, K_3}.
			\end{align*}
			Inductively, for $0 \leq s \leq B$
			\begin{align*}
				|\mathcal{F}^{i_{r}+s}(\phi(1))| =|s_i| 
				\leq  \varepsilon \left( (1+D_1) + (1+D_4)\sum_{k=0}^{s-1} \frac{1}{(\cos(k \sqrt{\varepsilon}))^2} \right),
			\end{align*}
			and hence, for  $i_r \leq i \leq i_{c}$,
			\begin{align*}
				|B_{m,f}(f^{(i_{r}+1)q_{m+1}+ q_m}(c_0))- z_{m}| &\leq \frac{L_1  \left[ (1+D_1)+(1+D_4)  D_5 \right]}{2(P+N)\, K_3}\\
				&\leq   \frac{L_1 \left[ (1+D_1)+(1+D_4)  D_5 \right]}{2\, K_3} \, \lambda^m,
			\end{align*}
			where $D_5= B \, \max_{0 \leq k \leq B} \{ \frac{1}{(\cos(k \sqrt{\varepsilon}))^{2}} \}$.  
			
			Putting together the estimatives that we get for points inside the Funnel and inside the Tunnel, we obtain the lemma for  $B_{m,f}(f^{jq_{m+1}+q_m}(c_0))$ with $N+P\leq j \leq i_c$.
			
			We can repeat the arguments above in Claim \ref{claimP} interchanging $B_{m,f}(f^{iq_{m+1}+ q_m}(c_0))$ by $B_{m,f}(f^{-jq_{m+1}}(\mathfrak{c}_{m}))$ and  $N+P \leq i \leq i_c$
			by $N+P \leq j \leq i_{\ell}$.
			Together those estimates give us the result for all  $v \in	\widehat{E}_{m+1} \cap I_m$ with $v \in [f^{-Pq_{m+1}}(\mathfrak{c}_{m}) , f^{q_m+Pq_{m+1}}(c_0)]$. 
			\textcolor{red}{Now, if $n > m$ note that every  $v \in \widehat{E}_{n+1} \cap I_m$ is between consecutive iterates of the form $f^{q_m+jq_{m+1}}(c_0)$ or  $f^{-jq_{m+1}}(\mathfrak{c}_{m})$. By an argument of continuity we extend the estimates for the rest endpoints of $\widehat{E}_{n+1}$ inside $I_m$.}
		\end{proof}
		
		%%%%%%%%%%%%%%%%%%%%%%%%%
		By Claim \ref{claimP} we can now estimate the difference between all these  endpoints and the center of the tubular, hence by Inequality \eqref{inq:estimativacentrofunnel}, we have  for $N+P \leq i \leq r(m)$,
		\begin{align*}
			| &B_{m,f}(f^{iq_{m+1}+q_m}(c_0))) - B_{m,g}(g^{iq_{m+1}+q_m}(c_0)))| \\
			&\leq |z_{m} - B_{m,f}(f^{iq_{m+1}+q_m}(c_0))| +|z_{m} - h(z_{m})| + |h(z_{m}) - B_{m,g}(g^{iq_{m+1}+q_m}(c_0)) | \\
			%&\leq \frac{2C}{P} + C\, \lambda^m\\
			&\leq C\, \lambda^m,
		\end{align*}
		and also $|B_{m,f}(f^{-jq_{m+1}}(\mathfrak{c}_{m}^f))-
		B_{m,g}(g^{-jq_{m+1}}(\mathfrak{c}_{m}^g))| \leq C\, \lambda^m$, \ for $-(N+P) \leq j\leq -2$.\\
		In particular, we have that  $| B_{m,f}(f^{iq_{m+1}+q_m}(c_0)) - B_{m,g}(g^{iq_{m+1}+q_m}(c_0))|< C\lambda^m$,  for $N+P \leq i \leq r(m)$, and  % \\
		%		&\leq S_1\, \left( \max_{v \in \widehat{E}_{n+1} \cap J_m} |B_{m+1,g}(g^{q_m}(c_0)) - B_{m+1,f}(f^{q_m}(c_0))| \right) + C\, \lambda^{m},
		%	\end{align*}
	\ $|B_{m,f}(f^{-jq_{m+1}}(\mathfrak{c}_{m}^f))-
	B_{m,g}(g^{-jq_{m+1}}(\mathfrak{c}_{m}^g))|<C\lambda^n$, \ for $-(N+P) \leq j\leq -2$, and hence they satisfy the lemma.
	
	%\begin{claim}\label{claimP}
	%There exists $C>0$ such that $|B_{m,f}(f^{jq_{m+1}+q_m}(c_0))-z_{m,f}|<C /P$  for $P+1 \leq j \leq r(m)$, moreover $|B_{m,f}(f^{-jq_{m+1}}(\mathfrak{c}_{m}^f))-z_{m,f}| < C/ P$ for $-P \leq j\leq -2$. 
	%\end{claim}
	Now, let us consider the points in $\widehat{E}_{m+2}$. We have two options: $m+1$ is not a two-bridge level or it is. In the first  case, all endpoints of $\widehat{E}_{m+2} \cap (J_m \setminus J_{m+1})$ are endpoints of $\widehat{E}_{m+1}$
	together with  the $r(m+1)$ and $\ell(m+1)$  images under $f^{q_{m+2}}$ of each endpoints in $\widehat{E}_{m+1} \cap E_{m+1}$ (except atmost one), and the images of $\mathfrak{c}_{m+1}^f$ under  $f^{q_m+jq_{m+1}}$  for $j\in \{0,1, \cdots, a_{n+1}-1\}$. By \eqref{eq:diferenciafreecriticalpoint}, we have $|B_{m+1,f}(\mathfrak{c}_{m+1}^f) - B_{m+1,g}(\mathfrak{c}_{m+1}^g)| \leq %C \lambda^{m+1/d} =
	(C\lambda^{1/d})(\lambda^{1/d})^m$, then $\mathfrak{c}_{m+1}^f$ satisfies Lemma \ref{lema_pasocero} for $\lambda_1=\lambda^{1/d}$. By the hypothesis of convergence of renormalizations we have that   $f^{q_m+jq_{m+1}}(\mathfrak{c}_{m+1}^f)$  for $j\in \{0,1, \cdots, a_{n+1}-1\}$ also satisfy the lemma. The endpoints in $\widehat{E}_{m+1} \cap E_{m+1}$ will also satisfy the lemma for an analogous argument used above for $m=n$. If $m+1$ is a two-bridge level then each endpoint in $\widehat{E}_{m+2}$ is the form  $f^{iq_{m+2}}(v)$ for $0 \leq i \leq r(n+1)-1$ or $0 \leq i \leq \ell(n+1)-1$, or is a backward iterates $f^{-jq_{m+2}}(v)$ for $ \ell(n+1) +1 \leq j \leq -1$ or $ r(n+1) +1 \leq j \leq -1$, for $v \in \widehat{E}_{m+1}$. Therefore we can repeat the argument above used for $m=n$. Inductively, we get the lemma for all $z  \in \widehat{E}_{n+1} \cap (J_m \setminus J_{m+1})$. We remark that if  $m$ is not a two-bridge level, then  $\widehat{E}_{m+1} \cap J_m$ is made of $\mathfrak{c}_{m}^f$ together with every (except at most one) point in $E_{n+1}$, therefore repeting a similar argument as the above but just with iterates of $c_0$ we get the lemma. Inductively, the proof also follows in this case.
	Now, by Claim \ref{claimP} and inequality \eqref{inq:estimativacentrofunnel}, we have  for $P+1 \leq i \leq r(m)$,
	\begin{align*}
		| &B_{m,f}(f^{iq_{m+1}+q_m}(c_0))) - B_{m,g}(g^{iq_{m+1}+q_m}(c_0)))| \\
		&\leq |z_{m,f} - B_{m,f}(f^{iq_{m+1}+q_m}(c_0))| +|z_{m,f} - z_{m,g}| + |z_{m,g} - B_{m,g}(g^{iq_{m+1}+q_m}(c_0)) | \\
		%&\leq \frac{2C}{P} + C\, \lambda^m\\
		&\leq C\, \lambda^m,
	\end{align*}
	and also $|B_{m,f}(f^{-jq_{m+1}}(\mathfrak{c}_{m}^f))-
	B_{m,g}(g^{-jq_{m+1}}(\mathfrak{c}_{m}^g))| \leq C\, \lambda^m$, \ for $-(N+P) \leq j\leq -2$.\\
	In particular, we have that  $| B_{m,f}(f^{iq_{m+1}+q_m}(c_0)) - B_{m,g}(g^{iq_{m+1}+q_m}(c_0))|< C\lambda^m$,  for $N+P \leq i \leq r(m)$, and  % \\
	%		&\leq S_1\, \left( \max_{v \in \widehat{E}_{n+1} \cap J_m} |B_{m+1,g}(g^{q_m}(c_0)) - B_{m+1,f}(f^{q_m}(c_0))| \right) + C\, \lambda^{m},
	%	\end{align*}
\ $|B_{m,f}(f^{-jq_{m+1}}(\mathfrak{c}_{m}^f))-
B_{m,g}(g^{-jq_{m+1}}(\mathfrak{c}_{m}^g))|<C\lambda^n$, \ for $-(N+P) \leq j\leq -2$, and hence they satisfy the lemma.

An analogous argument, using Claim \ref{claimP}, shows that the rest of the points in $\widehat{E}_{n+1}$ satisfy the lemma. 
%for $M+1 \leq i \leq r(m)$,
%{\small
	%	\begin{align*}
		%		| &B_{m,f}(f^{-kq_{m+2}}(c_0)) - B_{m,g}(g^{-kq_{m+2}}(c_0))| 
		%		&\leq C\, \lambda^m,
		%	\end{align*}
	%}
%and $| B_{m,f}(f^{-jq_{m+1}}(\mathfrak{c}_{m}^f)) - B_{m,g}(g^{-jq_{m+1}}(\mathfrak{c}_{m}^g))| 
%		\leq C\, \lambda^m$, \ for $-r(m) \leq j \leq -2$.
%and for $-r(m) \leq j  \leq 0$,
%{\small
	%\begin{align*}
	%	| B_{m,f}(f^{-jq_{m+1}}(\mathfrak{c}_{m}^f)) &- B_{m,g}(g^{-jq_{m+1}}(\mathfrak{c}_{m}^g))| \\ &\leq S_1\, \left( \max_{v \in \widehat{E}_{n+1} \cap J_m} |B_{m+1,g}(\mathfrak{c}_{m}^g) - B_{m+1,f}(\mathfrak{c}_{m}^f)| \right) + C\, \lambda^{m/d}.
	%\end{align*}
	%}
Now, if the forward iterates stopped early than the backward iterates (or viceversa) in the same tubular, then we can combine the previous arguments and get the lemma.
\end{proof}


